A Hybrid Approach for Trajectory Control Design

This work presents a methodology to design trajectory tracking feedback control laws, which embed non-parametric statistical models, such as Gaussian Processes (GPs). The aim is to minimize unmodeled dynamics such as undesired slippages. The proposed approach has the benefit of avoiding complex terramechanics analysis to directly estimate from data the robot dynamics on a wide class of trajectories. Experiments in both real and simulated environments prove that the proposed methodology is promising.

==> implementation_details.tex <==

\section{Implementation Details}

\subsection{Interception vs Trajectory Tracking Control Schemes}

\subsection{Geometric Saturation of g-Function Inputs}

==> notes.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








==> problem_statement.tex <==
\section{Problem Statement}\label{Sect:problem}

Let $\dot{{\bf z}}{=}{\bf s}({\bf z})$ be the non-linear system regulating the actual behavior of an embodied ground vehicle. 

%This system is very
%
%%Due to the complex dynamic effects between the robot and the environment, this system is quite difficult to be exactly derived.
%%
%%Statistical approaches are commonly employed to estimate 
%
%In many significant situations, a nominal model needs to capture strong linear effects that have to deal with uncertaity and noise
%
%nominal models for such systems are purely based on a theoretical hysical principle that can be unfeasbly complex and requires a large number of simplified assumptions. On the other hand,  
